Measurements of fiducial and differential cross-sections of $t\bar{t}$ production with additional heavy-flavour jets in proton-proton collisions at $\sqrt{s}$ = 13 TeV with the ATLAS detector

This paper presents measurements of $t\bar{t}$ production in association with additional $b$-jets in $pp$ collisions at the LHC at a centre-of-mass energy of 13 TeV. The data were recorded with the ATLAS detector and correspond to an integrated luminosity of 36.1 fb$^{-1}$. Fiducial cross-section measurements are performed in the dilepton and lepton-plus-jets $t\bar{t}$ decay channels. Results are presented at particle level in the form of inclusive cross-sections of $t\bar{t}$ final states with three and four $b$-jets as well as differential cross-sections as a function of global event properties and properties of $b$-jet pairs. The measured inclusive fiducial cross-sections generally exceed the $t\bar{t}b\bar{b}$ predictions from various next-to-leading-order matrix element calculations matched to a parton shower but are compatible within the total uncertainties. The experimental uncertainties are smaller than the uncertainties in the predictions. Comparisons of state-of-the-art theoretical predictions with the differential measurements are shown and good agreement with data is found for most of them.

==> tables/resultsdileptons/ObservableChi2_2b_nbjets_inc.tex <==
%%%% emu-channel total event yield summary%%%%
%\begin{table}
%\begin{center}
%\begin{tabular}{|l|c|c|}\hline
%Generators & \multicolumn{2}{|c|}{$N_{b\mathrm{-jets}}$} \\
%\hline
%             &  $\chi^{2}$/ndof & $p$-value \\
%\hline
%\ppyeight      &  16.89 / 2  &  $< 0.01$  \\
%\ppyeightradhi &  8.69 / 2  &  0.01  \\
%\ppyeightradlo &  22.57 / 2  &  $<0.01$  \\
%\amcnlopyeight &  12.65 / 2  &  $<0.01$  \\
%\phwseven      &  36.22 / 2  &  $0.01$ \\
%\sherpa        &  1.08 / 2  &  0.58 \\
%\textsc{Sherpa} $ttbb$ ME  &  0.05 / 1  &  0.83 \\
%\hline
%\end{tabular}
%\caption{Values of $\chi^{2}$/ndof and $p$-values between the unfolded normalised cross-section and the predictions for $b$-jet multiplicity measurements in the $e\mu$ channel. \ The number of degrees of freedom is equal to the number of bins minus one. The $\chi^{2}$/ndof and $p$-values for prediction from \textsc{Sherpa} $ttbb$ ME is computed only for $\ge$ 3$b$ selection.
%\label{tab:localchi2_nbjets}}
%\end{center}
%\end{table}

%table for generator systematics from aMC@NLO
%\begin{table}
%\begin{center}
%\begin{tabular}{lrrrr}
%  \toprule
%  Generators & \multicolumn{4}{c}{$N_{b\mathrm{-jets}}$}                     \\
%             & \multicolumn{2}{c}{$\ge 2 b$} & \multicolumn{2}{c}{$\ge 3 b$} \\
%
%                 & $\chi^2$ / NDF & $p$-value & $\chi^2$ / NDF & $p$-value \\
%  \midrule
%  \ppyeight      & 19.0 / 2       & $<0.01$   & 0.07 / 1       & 0.80      \\
%  \amcnlopyeight & 15.1 / 2       & $<0.01$   & $<0.01$ / 1    & 0.95      \\
%  \SHERPAtt      & 1.69 / 2       & 0.43      & 0.37 / 1       & 0.54      \\
%  \SHERPAttbb    & -              & -         & 0.37 / 1       & 0.54      \\
%  \phwseven      & 39.2 / 2       & $<0.01$   & 0.96 / 1       & 0.33      \\
%  \ppyeightradhi & 10.4 / 2       & 0.01      & 0.02 / 1       & 0.87      \\
%  \ppyeightradlo & 27.5 / 2       & $<0.01$   & 0.15 / 1       & 0.70      \\
%\hline
%\end{tabular}
%\caption{Values of $\chi^{2}$/ndof and $p$-values between the unfolded normalised cross-section and the predictions for $b$-jet multiplicity measurements in the $e\mu$ channel. \ The number of degrees of freedom is equal to the number of bins minus one. The $\chi^{2}$/ndof and $p$-values for prediction from \textsc{Sherpa} $ttbb$ ME is computed only for $\ge$ 3$b$ selection.
%\label{tab:localchi2_nbjets}}
%\end{center}
%\end{table}

%table for generator systematics from Sherpa
\begin{table}
\begin{center}
\begin{tabular}{lrrrr}
  \toprule
  Generators & \multicolumn{4}{c}{$N_{b\mathrm{-jets}}$}                     \\
             & \multicolumn{2}{c}{$\ge 2 b$} & \multicolumn{2}{c}{$\ge 3 b$} \\

                 & $\chi^2$ / NDF & $p$-value & $\chi^2$ / NDF & $p$-value \\
  \midrule
  \ppyeight      & 22.4 / 2       & $<0.01$   & 0.03 / 1       & 0.85      \\
  \amcnlopyeight & 17.9 / 2       & $<0.01$   & $<0.01$ / 1    & 0.97      \\
  \SHERPAtt      & 1.89 / 2       & 0.39      & 0.19 / 1       & 0.67      \\
  \SHERPAttbb    & -              & -         & 0.19 / 1       & 0.67      \\
  \powhelpyeight & -              & -         & 13.6 / 1       & $<0.01$      \\
  \phwseven      & 46.0 / 2       & $<0.01$   & 0.48 / 1       & 0.49      \\
  \ppyeightradhi & 12.3 / 2       & $<0.01$   & 0.01 / 1       & 0.91      \\
  \ppyeightradlo & 32.4 / 2       & $<0.01$   & 0.08 / 1       & 0.78      \\
\hline
\end{tabular}
\caption{Values of $\chi^{2}$/ndof and $p$-values between the unfolded normalised cross-section and the predictions for $b$-jet multiplicity measurements in the $e\mu$ channel. \ The number of degrees of freedom is equal to the number of bins minus one. The $\chi^{2}$/ndof and $p$-values for prediction from \textsc{Sherpa} $ttbb$ ME is computed only for $\ge$ 3$b$ selection.
\label{tab:localchi2_nbjets}}
\end{center}
\end{table}



==> tables/resultsdileptons/ObservableChi2_3b_HT_HThad.tex <==
% this table below is for generators systematics from aMC@NLO 
%\begin{table}
%\begin{center}
%\begin{tabular}{|l|c|c|c|c|}\hline
%Generators & \multicolumn{2}{|c|}{$H_{\mathrm{T}}$} & \multicolumn{2}{|c|}{$H_{\mathrm{T}^{\mathrm{had}}}$} \\
%\hline
%           &  $\chi^{2}$/ndof & $p$-value &  $\chi^{2}$/ndof & $p$-value  \\
%\hline
%\ppyeight      & 0.51 / 4 & 0.97    & 1.42 / 3  & 0.70    \\
%\amcnlopyeight & 4.06 / 4 & 0.40    & 3.38 / 3  & 0.34    \\
%\SHERPAtt      & 0.31 / 4 & 0.99    & 1.13 / 3  & 0.77    \\
%\SHERPAttbb    & 0.29 / 4 & 0.99    & 0.30 / 3  & 0.96    \\
%\phwseven      & 0.66 / 4 & 0.96    & 1.45 / 3  & 0.69    \\
%\ppyeightradhi & 3.12 / 4 & 0.54    & 4.26 / 3  & 0.24    \\
%\ppyeightradlo & 0.04 / 4 & $>0.99$ & 0.53 / 3  & 0.91    \\
%\hline
%\end{tabular}%\caption{Values of $\chi^{2}$/ndof and $p$-values between the unfolded normalised cross-section and the predictions for $H_{\mathrm{T}}$ and $H_{\mathrm{T}}^{\mathrm{had}}$ measurements in the di-lepton channel. \ The number of degrees of freedom is equal to the number of bins minus one. \label{tab:localchi2_HT}}
%\end{center}
%\end{table}


% this table below is for generators systematics from Sherpa
\begin{table}
\begin{center}
\begin{tabular}{|l|c|c|c|c|}\hline
Generators & \multicolumn{2}{|c|}{$H_{\mathrm{T}}$} & \multicolumn{2}{|c|}{$H_{\mathrm{T}^{\mathrm{had}}}$} \\
\hline
           &  $\chi^{2}$/ndof & $p$-value &  $\chi^{2}$/ndof & $p$-value  \\
\hline
\ppyeight      & 0.82 / 4 & 0.94    & 2.62 / 3  & 0.45   \\
\amcnlopyeight & 3.92 / 4 & 0.42    & 3.85 / 3  & 0.28    \\
\SHERPAtt      & 0.48 / 4 & 0.97    & 2.23 / 3  & 0.53   \\
\SHERPAttbb    & 0.29 / 4 & 0.99    & 0.32 / 3  & 0.96    \\
\powhelpyeight & 5.95 / 4 & 0.20    & 4.64 / 3  & 0.20    \\
\phwseven      & 0.37 / 4 & 0.99    & 2.36 / 3  & 0.50    \\
\ppyeightradhi & 3.92 / 4 & 0.42    & 6.32 / 3  & 0.10    \\
\ppyeightradlo & 0.10 / 4 & $>0.99$ & 1.05 / 3  & 0.79    \\
\hline
\end{tabular}
\caption{Values of $\chi^{2}$/ndof and $p$-values between the unfolded normalised cross-section and the predictions for
$H_{\mathrm{T}}$ and $H_{\mathrm{T}}^{\mathrm{had}}$ measurements in the di-lepton channel. \ The number of degrees of freedom is equal to the number of bins minus one. \label{tab:localchi2_HT}}
\end{center}
\end{table}


==> tables/resultsdileptons/ObservableChi2_3b_bjetpt.tex <==
% the table below for generator systematics from aMC@NLO+Py8  
%\begin{table}
%\begin{center}
%\begin{tabular}{|l|c|c|c|c|c|c|}\hline
%Generators & \multicolumn{2}{|c|}{$p_{\mathrm{T}}^{b_{1}}$} & \multicolumn{2}{|c|}{$p_{\mathrm{T}}^{b_{2}}$}  & \multicolumn{2}{|c|}{$p_{\mathrm{T}}^{b_{3}}$} \\
%\hline
%               &  $\chi^{2}$/ndof & $p$-value &  $\chi^{2}$/ndof & $p$-value &  $\chi^{2}$/ndof & $p$-value \\
%\hline
%\ppyeight      & 2.31 / 4 & 0.68 & 0.19 / 3 & 0.98 & 0.07 / 2 & 0.97   \\
%\amcnlopyeight & 2.50 / 4 & 0.65 & 0.13 / 3 & 0.99 & 0.41 / 2 & 0.82  \\
%\SHERPAtt      & 0.91 / 4 & 0.92 & 0.28 / 3 & 0.96 & 0.01 / 2 & $>0.99$  \\
%\SHERPAttbb    & 4.04 / 4 & 0.40 & 0.47 / 3 & 0.93 & 0.16 / 2 & 0.92     \\
%\phwseven      & 1.02 / 4 & 0.91 & 0.42 / 3 & 0.94 & 0.01 / 2 & $>0.99$  \\
%\ppyeightradhi & 3.27 / 4 & 0.51 & 0.31 / 3 & 0.96 & 0.24 / 2 & 0.89   \\
%\ppyeightradlo & 2.04 / 4 & 0.73 & 0.24 / 3 & 0.97 & 0.04 / 2 & 0.98   \\
%\hline
%\end{tabular}
%\caption{Values of $\chi^{2}$/ndof and $p$-values between the unfolded normalised cross-section and the predictions for $b$-jet $p_{\mathrm{T}}$ measurements. \ The number of degrees of freedom is equal to the number of bins minus one. \label{tab:localchi2_bjetspt}}
%\end{center}
%\end{table}


% the table below for generator systematics from Sherpa 
\begin{table}
\begin{center}
\begin{tabular}{|l|c|c|c|c|c|c|}\hline
Generators & \multicolumn{2}{|c|}{$p_{\mathrm{T}}^{b_{1}}$} & \multicolumn{2}{|c|}{$p_{\mathrm{T}}^{b_{2}}$}  & \multicolumn{2}{|c|}{$p_{\mathrm{T}}^{b_{3}}$} \\
\hline
               & $\chi^{2}$/ndof & $p$-value &  $\chi^{2}$/ndof & $p$-value &  $\chi^{2}$/ndof & $p$-value \\
\hline
\ppyeight      & 1.86 / 4 & 0.76 & 0.49 / 3 & 0.92 & 0.05 / 2 & 0.98   \\
\amcnlopyeight & 2.37 / 4 & 0.67 & 0.26 / 3 & 0.97 & 0.26 / 2 & 0.88  \\
\SHERPAtt      & 0.86 / 4 & 0.93 & 0.69 / 3 & 0.88 & $<0.01$ / 2 & $>0.99$  \\
\SHERPAttbb    & 3.35 / 4 & 0.50 & 0.64 / 3 & 0.89 & 0.13 / 2 & 0.94     \\
\powhelpyeight & 11.5 / 4 & 0.02 & 3.39 / 3 & 0.34 & 2.70 / 2 & 0.26  \\
\phwseven      & 1.01 / 4 & 0.91 & 1.04 / 3 & 0.79 & 0.01 / 2 & $>0.99$  \\
\ppyeightradhi & 2.47 / 4 & 0.65 & 0.53 / 3 & 0.91 & 0.18 / 2 & 0.91  \\
\ppyeightradlo & 1.73 / 4 & 0.79 & 0.65 / 3 & 0.89 & 0.03 / 2 & 0.99   \\
\hline
\end{tabular}
\caption{Values of $\chi^{2}$/ndof and $p$-values between the unfolded normalised cross-section and the predictions for
$b$-jet $p_{\mathrm{T}}$ measurements. \ The number of degrees of freedom is equal to the number of bins minus one. \label{tab:localchi2_bjetspt}}
\end{center}
\end{table}





==> tables/resultsdileptons/ObservableChi2_3b_dR_Ptbb_mbb.tex <==
% table for case of generator systematics from aMC@NLO
%\begin{table}[ht!]
%\begin{center}
%\begin{tabular}{|l|c|c|c|c|c|c|}\hline
%Generators & \multicolumn{2}{|c|}{$m_{b_1 b_2}$} & \multicolumn{2}{|c|}{$p_{\mathrm{T}, b_1 b_2}$}  & \multicolumn{2}{|c|}{$\Delta \mathrm{R}_{b_1 b_2}$} \\
%\hline
%               &  $\chi^{2}$/ndof & $p$-value &  $\chi^{2}$/ndof & $p$-value &  $\chi^{2}$/ndof & $p$-value \\
%\hline
%\ppyeight      & 0.27 / 4 & 0.99 & 1.02 / 3 & 0.80 & 1.93 / 4 & 0.75 \\
%\amcnlopyeight & 0.66 / 4 & 0.96 & 0.67 / 3 & 0.88 & 1.00 / 4 & 0.91 \\
%\SHERPAtt      & 0.63 / 4 & 0.96 & 0.34 / 3 & 0.95 & 1.61 / 4 & 0.81 \\
%\SHERPAttbb    & 1.56 / 4 & 0.82 & 0.44 / 3 & 0.93 & 3.64 / 4 & 0.46 \\
%\phwseven      & 0.42 / 4 & 0.98 & 0.32 / 3 & 0.96 & 2.69 / 4 & 0.61 \\
%\ppyeightradhi & 0.82 / 4 & 0.94 & 2.49 / 3 & 0.48 & 1.36 / 4 & 0.85 \\
%\ppyeightradlo & 0.17 / 4 & $>0.99$ & 0.52 / 3 & 0.91 & 1.81 / 4 & 0.77 \\
%\hline
%\end{tabular}%\caption{Values of $\chi^{2}$/ndof and $p$-values between the unfolded normalised cross-section and the predictions for $\Delta \mathrm{R}_{b_1 b_2}$, $p_{\mathrm{T}, b_1 b_2}$ and $m_{b_1 b_2}$ measurements in the di-lepton channel. \ The number of degrees of freedom is equal to the number of bins minus one. \label{tab:localchi2_dRbb_ptbb_mbb}}
%\end{center}
%\end{table}


% table for case of generator systematics from Sherpa
\begin{table}[ht!]
\begin{center}
\begin{tabular}{|l|c|c|c|c|c|c|}\hline
Generators & \multicolumn{2}{|c|}{$m_{b_1 b_2}$} & \multicolumn{2}{|c|}{$p_{\mathrm{T}, b_1 b_2}$}  & \multicolumn{2}{|c|}{$\Delta \mathrm{R}_{b_1 b_2}$} \\
\hline
               &  $\chi^{2}$/ndof & $p$-value &  $\chi^{2}$/ndof & $p$-value &  $\chi^{2}$/ndof & $p$-value \\
\hline
\ppyeight      & 1.52 / 4 & 0.82 & 1.51 / 3 & 0.68 & 1.05 / 4 & 0.90 \\
\amcnlopyeight & 1.75 / 4 & 0.78 & 1.03 / 3 & 0.79 & 5.05 / 4 & 0.28 \\
\SHERPAtt      & 0.26 / 4 & 0.99 & 0.58 / 3 & 0.90 & 0.78 / 4 & 0.94 \\
\SHERPAttbb    & 2.91 / 4 & 0.57 & 0.62 / 3 & 0.89 & 3.97 / 4 & 0.41 \\
\powhelpyeight & 9.95 / 4 & 0.04 & 5.29 / 3 & 0.15 & 1.03 / 4 & 0.90 \\
\phwseven      & 0.45 / 4 & 0.98 & 0.42 / 3 & 0.94 & 1.31 / 4 & 0.86 \\
\ppyeightradhi & 3.70 / 4 & 0.45 & 3.16 / 3 & 0.37 & 0.79 / 4 & 0.94 \\
\ppyeightradlo & 1.02 / 4 & 0.91 & 0.82 / 3 & 0.84 & 1.56 / 4 & 0.82 \\
\hline
\end{tabular}
\caption{Values of $\chi^{2}$/ndof and $p$-values between the unfolded normalised cross-section and the predictions for $\Delta \mathrm{R}_{b_1 b_2}$, $p_{\mathrm{T}, b_1 b_2}$ and $m_{b_1 b_2}$ measurements in the di-lepton channel. \ The number of degrees of freedom is equal to the number of bins minus one. \label{tab:localchi2_dRbb_ptbb_mbb}}
\end{center}
\end{table}

